Duality of Session Types: The Final Cut

Duality is a central concept in the theory of session types. Since a flaw was found in the original definition of duality for recursive types, several other definitions have been published. As their connection is not obvious, we compare the competing definitions, discuss tradeoffs, and prove some equivalences. Some of the results are mechanized in Agda.

==> eptcsdata.tex <==
\providecommand{\firstpage}{23}
\providecommand{\publicationstatus}{S. Balzer, L. Padovani (Eds.): Programming Language Approaches\\
to Concurrency- \& Communication-cEntric Software (PLACES 2020)\\
EPTCS 314, 2020, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.314.3}{10.4204/EPTCS.314.3}}

